How Well Do Deep Learning Models Capture Human Concepts? The Case of the Typicality Effect

How well do representations learned by ML models align with those of humans? Here, we consider concept representations learned by deep learning models and evaluate whether they show a fundamental behavioral signature of human concepts, the typicality effect. This is the finding that people judge some instances (e.g., robin) of a category (e.g., Bird) to be more typical than others (e.g., penguin). Recent research looking for human-like typicality effects in language and vision models has focused on models of a single modality, tested only a small number of concepts, and found only modest correlations with human typicality ratings. The current study expands this behavioral evaluation of models by considering a broader range of language (N = 8) and vision (N = 10) model architectures. It also evaluates whether the combined typicality predictions of vision + language model pairs, as well as a multimodal CLIP-based model, are better aligned with human typicality judgments than those of models of either modality alone. Finally, it evaluates the models across a broader range of concepts (N = 27) than prior studies. There were three important findings. First, language models better align with human typicality judgments than vision models. Second, combined language and vision models (e.g., AlexNet + MiniLM) better predict the human typicality data than the best-performing language model (i.e., MiniLM) or vision model (i.e., ViT-Huge) alone. Third, multimodal models (i.e., CLIP ViT) show promise for explaining human typicality judgments. These results advance the state-of-the-art in aligning the conceptual representations of ML models and humans. A methodological contribution is the creation of a new image set for testing the conceptual alignment of vision models.

==> cv_table.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{category} & \textbf{supercategory} & \textbf{alexnet} & \textbf{convnext\_base} & \textbf{densenet161} & \textbf{efficientnet\_v2\_m} & \textbf{inception\_v3} & \textbf{mobilenet\_v2} & \textbf{resnet50} & \textbf{swin\_b} & \textbf{vgg19} & \textbf{vit\_b\_16} & \textbf{vit\_h\_14} & \textbf{vit\_l\_16} & \textbf{category\_avg} & \textbf{category\_max} \\ \hline
        \textbf{ship} & vehicle & -0.2107597856465369 & -0.1051858230390635 & -0.0958704733972276 & -0.160689781321669 & -0.2274497870881595 & -0.0916009381447195 & -0.2181344374463236 & -0.1210995453438665 & -0.2456923468034215 & -0.0714176805874084 & 0.3247254580313682 & 0.1263804632319702 & -0.06870180362874774 & 0.3247254580313682 \\ \hline
        \textbf{vehicle} & vehicle & 0.1207192270777382 & 0.1285496634287267 & 0.1722695997217454 & 0.1735746724469102 & 0.0287115999536242 & 0.0874398725860374 & 0.012398190889065 & -0.0261014545032947 & 0.1866253996985575 & 0.0287115999536242 & 0.0849238648593955 & 0.5156688249346566 & 0.14123106429552343 & 0.5156688249346566 \\ \hline
        \textbf{flower} & plant & -0.2730027504367756 & -0.2352951882217513 & -0.1711923324562101 & -0.3076937076745979 & 0.0120664199088077 & -0.4351452679613799 & -0.2277536757787465 & -0.2586738767950663 & -0.1659132737461067 & -0.1221725015766785 & 0.1067579518067511 & 0.5096061851619494 & -0.05041245010269236 & 0.5096061851619494 \\ \hline
        \textbf{fruit} & plant & -0.1065680831566127 & -0.084819494757304 & -0.3405828943331745 & -0.1043932243166818 & -0.3340583178133819 & -0.3362331766533128 & -0.2857764515669166 & -0.3066550964302529 & -0.1209221515001564 & -0.2287951499607277 & 0.2540611322553524 & 0.1516310660115968 & -0.12398051560165682 & 0.2729359188208742 \\ \hline
        \textbf{tree} & plant & -0.164694841330123 & -0.2285140923455456 & -0.0672503935431335 & -0.0816611921595193 & -0.1180313029532548 & -0.1684690981106049 & -0.1794487541992799 & -0.1557738707580747 & -0.1499409284609661 & -0.1640086128245808 & 0.1352658178848778 & 0.3089371926198845 & -0.03382121152719138 & 0.3567030428503903 \\ \hline
        \textbf{vegetable} & plant & -0.1532243250591514 & -0.3006738639979832 & -0.252165660587297 & -0.4319540017999195 & -0.2105872005209946 & -0.2540905892940703 & -0.1640039258170817 & -0.2694900189482563 & -0.1486044961628956 & -0.3445622385124135 & 0.1860281851526578 & 0.1904302782161468 & -0.14024710024863005 & 0.1904302782161468 \\ \hline
        \textbf{color} & abstract & 0.1526965884399176 & -0.0506822719077173 & 0.2209227237003064 & 0.0344379539885771 & 0.3190384039319131 & 0.2378168143362122 & 0.2248213600009 & -0.1104613618501532 & 0.4197531750305822 & 0.3502274943366623 & 0.0038813956840982 & 0.2032850729805424 & 0.1726716984142549 & 0.4297865470535702 \\ \hline
        \textbf{flying thing} & abstract & 0.2283708613640793 & 0.2283708613640793 & 0.1194555274827492 & 0.2766800820372501 & -0.1510761082870063 & 0.1264823232170286 & 0.0281071829371174 & 0.132630769484523 & 0.3293810500443453 & 0.1826966890912635 & 0.2048964178508639 & -0.0772397741135559 & 0.10946409067907857 & 0.3293810500443453 \\ \hline
        \textbf{green thing} & abstract & 0.0341763680447471 & -0.0842758166557969 & 0.0333996324073665 & -0.0846641844744872 & -0.3732214737613866 & -0.1635028516686199 & -0.1335985296294661 & -0.0838874488371066 & -0.2640901167094099 & -0.1518518171079106 & 0.423344108091338 & 0.0841771907731256 & -0.03033400221319819 & 0.423344108091338 \\ \hline
        \textbf{bird} & animal & 0.279093334459073 & -0.0719485214732622 & 0.0043503757169879 & -0.000167322142961 & -0.107253493638049 & 0.0528737971756996 & -0.0572241728926876 & -0.0369781935943975 & 0.2421151408646754 & -0.0640843807540916 & 0.4240049163406393 & -0.0304526300189156 & 0.07635941267539881 & 0.4360415045565612 \\ \hline
        \textbf{fish} & animal & 0.1900586705346386 & 0.0492858789068754 & 0.0064687716065274 & 0.0591430546882505 & -0.1838979356712791 & -0.0489778421637075 & 0.0040044776611836 & 0.1115093010268057 & 0.1980676258570058 & 0.1484737102069624 & 0.1579847781659369 & 0.1783532742942556 & 0.0594923773176402 & 0.1980676258570058 \\ \hline
        \textbf{four-legged animal} & animal & -0.0621336308067587 & 0.1137429984149786 & 0.0087027561064841 & 0.0305608412111419 & 0.1936869207884956 & 0.0835869365576266 & 0.0862180023572613 & -0.0607169030684939 & -0.0953255378175354 & -0.1171836229221932 & 0.0967121986315013 & 0.0453352876244754 & 0.014540996288003606 & 0.1936869207884956 \\ \hline
        \textbf{snake} & animal & 0.0193748769371471 & -0.1664478064145819 & -0.1532376630483453 & -0.1365048147844455 & -0.2280951421236864 & -0.0801415364218357 & -0.1549990154971768 & -0.221930408552776 & -0.0598859832602728 & -0.2369019043678442 & 0.064995752808442 & -0.206078236513292 & -0.12035056465040772 & 0.064995752808442 \\ \hline
        \textbf{insect} & animal & 0.3394631832298267 & -0.1267329217391353 & -0.0011315439440994 & -0.0616691449534185 & -0.2806228981366568 & 0.0492221615683248 & -0.2432819479813758 & -0.076379216226711 & 0.15671883625777 & -0.1465349407608752 & 0.1489588021947051 & -0.1318248694875827 & -0.01841651755064553 & 0.3394631832298267 \\ \hline
        \textbf{fabric} & garment & 0.3271854993800907 & 0.3653161402852893 & 0.4501875668162151 & 0.1943432665490764 & 0.5227587866035285 & 0.1599026876669616 & 0.3554759748903994 & 0.4932382904188586 & 0.4538776288392988 & 0.4526476081649376 & -0.2078395889621235 & 0.2200414397291309 & 0.2848249021759711 & 0.5227587866035285 \\ \hline
        \textbf{footwear} & garment & 0.3778496595918033 & 0.2486176913275057 & 0.1218472843634805 & 0.1243088456637528 & 0.1809247555700165 & 0.0603082518566721 & 0.3323107755367651 & 0.155078361917157 & 0.1870786588206974 & 0.0 & -0.064498004813667 & 0.2063135844032729 & 0.1529292335083222 & 0.3778496595918033 \\ \hline
        \textbf{clothing} & garment & 0.3103508406689849 & 0.1515826046486883 & 0.2309667226588366 & -0.0037639021470328 & 0.1522669504936034 & 0.2388366998753599 & 0.0872540952266716 & 0.1283148459215758 & 0.2251497829770585 & 0.0893071327614168 & 0.180368233933006 & 0.0767730805302607 & 0.1362675346995102 & 0.3103508406689849 \\ \hline
        \textbf{instrument} & man-made misc & 0.3505397073367767 & 0.1910634009220233 & 0.1995379872532421 & 0.533898938866783 & 0.0019260423480042 & 0.1298152542554876 & 0.023497716645652 & 0.3547770005023861 & 0.4884443394538822 & 0.1922190263308258 & 0.5138783081814113 & 0.282904755103086 & 0.27889809065829496 & 0.533898938866783 \\ \hline
        \textbf{toy} & man-made misc & 0.2291114284788016 & 0.0808336858052914 & 0.1279453431764736 & 0.1175311873365281 & 0.1735692639990921 & 0.1686101421705466 & -0.0540544279311458 & 0.106621119313728 & 0.1403431477478373 & 0.046119833005473 & 0.2762213235515494 & 0.0086154645509531 & 0.11507198080900703 & 0.2762213235515494 \\ \hline
        \textbf{furniture} & man-made misc & 0.1319371086475387 & 0.1126844833513313 & -0.0266139232035807 & 0.2015863119249947 & 0.0152888494999293 & 0.2672717394061727 & 0.1211782886290698 & 0.1540210023696589 & 0.0317102063702239 & 0.2106463708879158 & 0.2411182525102441 & 0.1194183499376799 & 0.10742446275879627 & 0.2672717394061727 \\ \hline
        \textbf{earth formation} & environment & 0.4473142882756512 & 0.0971074898335132 & 0.1002066650409657 & 0.203512505289384 & -0.1342975923229437 & 0.1590909939825641 & 0.27169435985334 & 0.1219008914931335 & 0.1446281763477856 & 0.3884299593340528 & -0.0791858806515509 & 0.0448343174568268 & 0.13291091166409047 & 0.4473142882756512 \\ \hline
        \textbf{dwelling} & environment & -0.0475106992474414 & 0.1308171308045989 & 0.0728931276125128 & 0.031239911833934 & 0.2030594269205714 & 0.0462090362543608 & -0.042304047275119 & 0.1295154678115183 & -0.0637814866609487 & 0.1503420757008077 & 0.0382775155827833 & 0.1475627104198666 & 0.07915244503329225 & 0.2371543560319286 \\ \hline
        \textbf{weather} & environment & 0.6284982694256935 & 0.02472353440805 & 0.1392325358769134 & -0.1437868711626069 & 0.1906314626725964 & 0.2973330322231283 & 0.3532862943045048 & 0.0461939721834619 & 0.3077429414475704 & 0.0065061932652763 & -0.0494084523990369 & -0.0155347127476123 & 0.11490791728527491 & 0.6284982694256935 \\ \hline
        \textbf{carpenters tool} & man-made tool & 0.0269938853505179 & 0.1202454892886706 & 0.1202454892886706 & -0.0944785987268126 & 0.0846626404175334 & 0.2650308743505394 & 0.1582823277371277 & 0.1300614475979499 & 0.1631903068917673 & 0.0785276664742339 & -0.0935515351491804 & -0.1500760976157965 & 0.04648300961443709 & 0.2650308743505394 \\ \hline
        \textbf{gardeners tool} & man-made tool & 0.0232767177921893 & 0.4100283364931818 & 0.0017905167532453 & 0.4422576380515978 & 0.3169214653244244 & 0.3670559344152937 & 0.1432413402596268 & 0.4923921071424672 & 0.005371550259736 & 0.5031352076619393 & 0.2871902358906028 & -0.1848630013941241 & 0.205869872926844 & 0.5031352076619393 \\ \hline
        \textbf{kitchen utensil} & man-made tool & 0.456429887579833 & 0.3929137543567494 & 0.2865611591925164 & 0.3028094723426076 & 0.2732670847969874 & 0.5509655277258177 & 0.4859722751254532 & 0.5553968858576608 & 0.5480112889712557 & 0.5376714533302887 & 0.1353729512803809 & -0.2048392089043404 & 0.31088872551163726 & 0.5553968858576608 \\ \hline
        \textbf{weapon} & man-made tool & 0.1257792121342098 & 0.1814601281778125 & 0.0740755043794358 & 0.3166852099979907 & 0.0795441657765753 & 0.0507094056825668 & 0.0596581243324315 & 0.1914031488998844 & 0.0293319111301121 & 0.1387051390729033 & 0.1554980190401043 & -0.3503370246327333 & 0.042703198817960655 & 0.3166852099979907 \\ \hline
        \textbf{model\_avg} & all & 0.14004909255799478 & 0.05825064708389721 & 0.05122275572746692 & 0.0530053017246158 & 0.014804925432922382 & 0.06742222906993149 & 0.03654894075449073 & 0.05832989692712293 & 0.10901425355142401 & 0.06877238185940221 & 0.14629563547231297 & 0.07663048083524918 & N/A & N/A \\ \hline
        \textbf{model\_max} & all & 0.6284982694256935 & 0.4100283364931818 & 0.4501875668162151 & 0.533898938866783 & 0.5227587866035285 & 0.5509655277258177 & 0.4859722751254532 & 0.5553968858576608 & 0.5480112889712557 & 0.5376714533302887 & 0.5138783081814113 & 0.5156688249346566 & N/A & N/A \\ \hline
    \end{tabular}
\end{table}

==> nlp_table.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
    \hline
        \textbf{category} & \textbf{supercategory} & \textbf{all-MiniLM-L12-v2} & \textbf{all-mpnet-base-v2} & \textbf{all-roberta-large-v1} & \textbf{glove-twitter-200} & \textbf{sentence-t5-base} & \textbf{sentence-t5-large} & \textbf{sentence-t5-xl} & \textbf{sentence-t5-xxl} & \textbf{text-embedding-ada-002} & \textbf{word2vec-google-news-300} & \textbf{xlnet\_base\_cased} & \textbf{category\_avg} & \textbf{category\_max} \\ \hline
        \textbf{color} & abstract & 0.712800670291871 & 0.6257311262452797 & 0.5289149914472042 & 0.330628554491084 & 0.4117878540033124 & 0.4541911290191593 & 0.4587832872946166 & 0.2014640296012463 & 0.6010397630081866 & 0.1209739093608571 & 0.0180996298632116 & 0.4058559040569117 & 0.712800670291871 \\ \hline
        \textbf{flying thing} & abstract & 0.4637685184624381 & 0.231884259231219 & 0.0851998982781373 & 0.6357878378986938 & 0.26382528127862 & 0.4804571583313516 & 0.3168878848440568 & 0.2975473097127294 & 0.5129560886023937 & 0.3970593619435156 & 0.6842105910422523 & 0.3972349263295825 & 0.6842105910422523 \\ \hline
        \textbf{green thing} & abstract & 0.3402102091727104 & 0.1165103456070926 & 0.349919404639968 & 0.610204875838364 & 0.6160840094786356 & 0.1184521847005441 & 0.6075902042008972 & 0.5158571072013208 & 0.5456567852598836 & 0.1147549467994535 & 0.383258620345307 & 0.39259079029492516 & 0.6160840094786356 \\ \hline
        \textbf{flower} & plant & 0.3785839246388435 & 0.4366535704499809 & 0.604829297928989 & -0.0501985447916993 & 0.073789065045834 & 0.4012084619678581 & 0.1079227822098933 & 0.1412198886591472 & 0.5377098371862459 & 0.2509927239584966 & 0.5767086405492686 & 0.3144926952548053 & 0.604829297928989 \\ \hline
        \textbf{fruit} & plant & 0.6324489506518977 & 0.5041322790959761 & 0.3797303534519303 & 0.5838766751553021 & 0.491010568609747 & 0.5480644276625798 & 0.4799212458557 & 0.3021840450477803 & 0.3536320473727598 & 0.2953329694099493 & -0.1496933642165084 & 0.40187638164519207 & 0.6324489506518977 \\ \hline
        \textbf{tree} & plant & 0.4594299844604889 & 0.4017867899949459 & 0.3287034541547038 & 0.1177914997113508 & 0.5112363238367189 & 0.3129201985272337 & 0.2515703683804598 & 0.2301170626295919 & 0.4402155863053079 & -0.1300614475979499 & 0.1718896083115522 & 0.2814181298831277 & 0.5112363238367189 \\ \hline
        \textbf{vegetable} & plant & 0.7187683791091352 & 0.6675652755089665 & 0.4211744010419892 & -0.0787827371427947 & 0.1893453882493922 & 0.6244468724772455 & 0.3813328051720318 & 0.0995164133589829 & 0.3353225807199019 & 0.2435102784413656 & 0.3495417046386714 & 0.35924921468862614 & 0.7187683791091352 \\ \hline
        \textbf{instrument} & man-made misc & 0.5959175024725204 & 0.5855168737932974 & 0.4171807725777244 & 0.4443118146991563 & 0.6489404519410188 & 0.2211096615508899 & 0.7140042287267357 & 0.6919391218167968 & 0.3551622089719869 & 0.456619621200518 & 0.0148963852624107 & 0.4677816948193687 & 0.7140042287267357 \\ \hline
        \textbf{toy} & man-made misc & 0.3838360295294208 & 0.3754055224208935 & 0.4180539701463848 & 0.3018708660529717 & 0.3635008997528338 & 0.3025064315412748 & 0.7677259666978937 & 0.625191381525102 & 0.5683153615513131 & 0.2409709380684098 & 0.3859649937587706 & 0.43030385100411533 & 0.7677259666978937 \\ \hline
        \textbf{fabric} & man-made misc & 0.7589227560808872 & 0.6482208953883752 & 0.1746629357592966 & 0.1843662949946685 & 0.3701609745562344 & 0.0787213231591195 & 0.5919965762291833 & 0.673336296842598 & 0.2410840521748037 & -0.0729702388610477 & 0.2187090172294452 & 0.3515646257775968 & 0.7589227560808872 \\ \hline
        \textbf{footwear} & man-made misc & 0.5271914494474023 & 0.5064766577205888 & 0.3604373760465539 & 0.6962562988753879 & 0.2816968015250646 & 0.5737997308327325 & 0.2480716047534978 & 0.517073178926032 & 0.4194745324679723 & 0.3203953540279433 & 0.12583117325566 & 0.4160640143526215 & 0.6962562988753879 \\ \hline
        \textbf{clothing} & man-made misc & 0.2459142308717094 & 0.4062930770923895 & 0.5150452090058412 & 0.6895231605855279 & 0.4773823192797684 & 0.6066902639890868 & 0.6787298620082515 & 0.6868145625766992 & 0.4212617694063196 & 0.3990759745064843 & 0.174274666216013 & 0.4819095541398264 & 0.6895231605855279 \\ \hline
        \textbf{furniture} & man-made misc & 0.4660267829052547 & 0.6223128000156438 & 0.5990963989231586 & 0.6099719849110953 & -0.0182425597152619 & 0.5849400567935943 & 0.1898002489524062 & 0.2689807209080112 & 0.4462079039238647 & -0.1438145330278191 & -0.3973946448126628 & 0.29344410543429866 & 0.6223128000156438 \\ \hline
        \textbf{bird} & animal & 0.1579521029552547 & 0.1154522786431416 & 0.3523804330760237 & 0.6211604405524279 & 0.5096308991768304 & 0.4173014245449208 & 0.6003334535757796 & 0.6394856353307217 & 0.3997325995340079 & 0.6371507093191241 & 0.0188752150104418 & 0.40631410833806125 & 0.6394856353307217 \\ \hline
        \textbf{fish} & animal & 0.6154574128496076 & 0.753457873788859 & 0.5107249201724973 & 0.2858641258300256 & 0.3521475043453926 & 0.3859700391894686 & 0.4159512333557076 & 0.0134969426752589 & 0.2800053995396864 & 0.1108241357384519 & 0.2568825107186563 & 0.3618892816548738 & 0.753457873788859 \\ \hline
        \textbf{four-legged animal} & animal & 0.709375817516904 & 0.6359083648040265 & 0.6618142434465838 & 0.5410113079177606 & 0.1289172062336641 & 0.5523214282463998 & 0.2632059627270643 & 0.5299929589606193 & 0.739531879374256 & 0.3537499122353286 & 0.5977900477395643 & 0.519419920836561 & 0.739531879374256 \\ \hline
        \textbf{snake} & animal & 0.1514763105995137 & 0.1488342819262664 & 0.1814193022296502 & 0.4263890249424749 & 0.7766225902359215 & 0.2245724372260233 & 0.7926227386876917 & 0.7643147837345599 & -0.1144879091740511 & -0.0390715042775972 & 0.6721949915350964 & 0.36226245887868636 & 0.7926227386876917 \\ \hline
        \textbf{insect} & animal & 0.6794921384317033 & 0.7451216871894697 & 0.5635088841615123 & 0.5746632481569696 & 0.4709886516791648 & 0.6195203093944339 & 0.199786814107627 & 0.1848904288452162 & 0.4090531357919412 & 0.0098039661759063 & 0.5009929672417435 & 0.4507111119250626 & 0.7451216871894697 \\ \hline
        \textbf{carpenters tool} & man-made tool & 0.3226996294175549 & 0.347239525190753 & 0.0404908280257768 & 0.5972162374450175 & 0.1652893443974692 & 0.4564420613814846 & 0.2675621262434033 & 0.2871902358906028 & 0.1521473537938281 & 0.1296215868598799 & 0.4009076091092592 & 0.28789150343227543 & 0.5972162374450175 \\ \hline
        \textbf{gardeners tool} & man-made tool & 0.2291861444154029 & 0.0823637706492854 & 0.0662491198700774 & 0.252532090039522 & 0.5792400319208609 & 0.0984784214284934 & 0.1164988378807124 & 0.4080713483307638 & 0.5783369112982434 & 0.2703740311836186 & 0.1611571107875325 & 0.2584079834367739 & 0.5792400319208609 \\ \hline
        \textbf{kitchen utensil} & man-made tool & 0.5193894343574625 & 0.765545564384696 & 0.566159099062637 & 0.6698751899570945 & 0.2530909180192492 & 0.6547753058724409 & 0.258946491957998 & 0.3070923221210428 & 0.3716957563411225 & 0.2429260027947853 & 0.1783278300520403 & 0.43525671953823347 & 0.765545564384696 \\ \hline
        \textbf{weapon} & man-made tool & 0.4429483970675679 & 0.3986973702586417 & 0.3172053802936886 & 0.1394628843353647 & 0.6939572615056685 & 0.5104202597267228 & 0.6010397630081866 & 0.7816765782690254 & 0.3233391859899754 & 0.0888430226136397 & 0.4066370790797706 & 0.42765701655893196 & 0.7816765782690254 \\ \hline
        \textbf{earth formation} & environment & 0.1435951179453014 & -0.0702479713689244 & 0.1373967675303963 & 0.2668409135815202 & 0.3012738671072278 & -0.0609504457465667 & 0.3328944479114849 & 0.6798424872915287 & -0.0609504457465667 & 0.1880903025001447 & 0.2496446372979237 & 0.19158451620940636 & 0.6798424872915287 \\ \hline
        \textbf{dwelling} & environment & 0.5733825484519982 & 0.0950213984948828 & 0.4627411940401484 & 0.3025379868353494 & -0.2295253808459724 & 0.2746508915400037 & 0.3860376117781668 & 0.2299137486646627 & 0.3970072128895788 & 0.2238130483255057 & 0.4306353669488246 & 0.2860196024657408 & 0.5733825484519982 \\ \hline
        \textbf{weather} & environment & 0.178920314795099 & 0.0396877789181856 & 0.1977882752644004 & 0.7738793056678381 & 0.5768796962754232 & 0.3077429414475704 & 0.7109519497807988 & 0.6100902544831768 & 0.1587511156727424 & 0.5445095366495788 & -0.1959132072343404 & 0.35484436015640664 & 0.7738793056678381 \\ \hline
        \textbf{ship} & vehicle & 0.0143611640311636 & 0.1486574547009643 & 0.233271880614307 & 0.5076859918016842 & 0.4536539388172145 & -0.1412828029011776 & 0.6173007934590407 & 0.6328368872541508 & 0.0329918633148354 & 0.1080369844145452 & -0.1708511875366608 & 0.22151481527000613 & 0.6328368872541508 \\ \hline
        \textbf{vehicle} & vehicle & 0.1566087270197686 & 0.4672160356089763 & -0.0104405818013179 & 0.3231220251503368 & 0.5306248683529928 & 0.7497642806071421 & 0.7432413959141231 & 0.4212617694063196 & 0.2394808450677295 & 0.5211896126823943 & 0.397737696350947 & 0.4127096976690375 & 0.7497642806071421 \\ \hline
        \textbf{model\_avg} & all & 0.42883943140551406 & 0.4000535142871805 & 0.3505058596069727 & 0.42066108716638867 & 0.37938180648381575 & 0.38360127601889 & 0.4481744698412374 & 0.43486657407643287 & 0.35869160817178775 & 0.21787782242390674 & 0.23930798846459964 & N/A & N/A \\ \hline
        \textbf{model\_max} & all & 0.7589227560808872 & 0.765545564384696 & 0.6618142434465838 & 0.7738793056678381 & 0.7766225902359215 & 0.7497642806071421 & 0.7926227386876917 & 0.7816765782690254 & 0.739531879374256 & 0.6371507093191241 & 0.6842105910422523 & N/A & N/A \\ \hline
    \end{tabular}
\end{table}
